Structure Pretraining and Prompt Tuning for Knowledge Graph Transfer

Knowledge graphs (KG) are essential background knowledge providers in many tasks. When designing models for KG-related tasks, one of the key tasks is to devise the Knowledge Representation and Fusion (KRF) module that learns the representation of elements from KGs and fuses them with task representations. While due to the difference of KGs and perspectives to be considered during fusion across tasks, duplicate and ad hoc KRF modules design are conducted among tasks. In this paper, we propose a novel knowledge graph pretraining model KGTransformer that could serve as a uniform KRF module in diverse KG-related tasks. We pretrain KGTransformer with three self-supervised tasks with sampled sub-graphs as input. For utilization, we propose a general prompt-tuning mechanism regarding task data as a triple prompt to allow flexible interactions between task KGs and task data. We evaluate pretrained KGTransformer on three tasks, triple classification, zero-shot image classification, and question answering. KGTransformer consistently achieves better results than specifically designed task models. Through experiments, we justify that the pretrained KGTransformer could be used off the shelf as a general and effective KRF module across KG-related tasks. The code and datasets are available at https://github.com/zjukg/KGTransformer.

==> secs/impact.tex <==
\section{Broader Impact}

==> secs/preliminary.tex <==
\section{Preliminary}
\paragraph{Knowledge Graph (KG).}
A KG formulated as $\mathcal{G}=\{ \mathcal{E}, \mathcal{R}, \mathcal{T}\}$ includes a set of entities $\mathcal{E}$, relations $\mathcal{R}$, and a set of triples $\mathcal{T} = \{(h,r,t) | h,t\in\mathcal{E}; r\in\mathcal{R}\}$, where the head entity $h$ is related to the tail entity $t$ via the relation $r$. A triple instance is like (\textit{William Shakespeare, field of work, Fiction}).

\paragraph{Transformer.} Transformer layer \cite{transformer} includes a self-attention module and a position-wise feed-forward network. Suppose the input of self-attention module is $H=[ s_1^{\top}, ..., s_n^{\top}]^\top \in \mathbb{R}^{n\times d}$ with the $i$th row as the $d$ dimensional hidden state for the $i$th element. The self-attention operation $Attn()$ is 
\begin{align}
    &Q = HW_{Q}, \; K = HW_{K}, \; V=HW_{V}, \nonumber \\
    & A = \frac{QK^{\top}}{\sqrt{d_K}}, \;Attn(H) = selftmax(A)V, 
    \label{equ:transformer}
\end{align}
where $W_{Q}\in \mathbb{R}^{d\times d_Q}$,$W_{K}\in \mathbb{R}^{d\times d_K}$,$W_{V}\in \mathbb{R}^{d\times d_V}$ is the projection matrix to generate the query, key, and value representation of $H$; $A$ is the matrix capturing similarity between the query and the key. 
% In this paper, we consider $d_{Q}=d_{K}=d_{V}=d$ for simplicity. 
 


==> tables/res-qa-error-bar.tex <==
\begin{table}[!hbpt]
% \begin{wraptable}{r}{0.5\textwidth}
% \renewcommand\arraystretch{1.1}
\centering
% \vspace{-5mm}
\caption{Accuracy with error bar of QA on CommonsenseQA. 
% Results of baselines are taken from \cite{qagnn}
}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
& \textbf{IHdev} & \textbf{IHtest} \\
\midrule
% RoBERTa-large\cite{roberta} & 73.07 ($\pm$.45) & 68.69 ($\pm$.56) \\ 
% \midrule
% + RGCN\cite{rgcn}   & 72.69 ($\pm$.19) & 68.41 ($\pm$.66) \\
% + GconAttn\cite{DBLP:conf/aaai/WangKMYTACFMMW19} & 72.61 ($\pm$.39) & 68.59 ($\pm$.96) \\
% + KagNet\cite{DBLP:conf/emnlp/LinCCR19}   & 73.47 ($\pm$.22) & 69.01 ($\pm$.76) \\
% + RN\cite{DBLP:conf/nips/SantoroRBMPBL17}       & 74.57 ($\pm$.91) & 69.08 ($\pm$.21) \\
% + MHGRN\cite{DBLP:conf/emnlp/FengCLWYR20}    & 74.45 ($\pm$.10) & 71.11 ($\pm$.81) \\
% + QA-GNN\cite{qagnn}   & 76.54 ($\pm$.21) & 73.41 ($\pm$.92) \\
% + GREASELM\cite{greaselm} & 78.50 ($\pm$.50) & 74.20 ($\pm$.40) \\
% + MorsE\cite{morse} & 77.67 ($\pm$.34) & 75.56 ($\pm$.21) \\
RoBERTa-L \cite{roberta} & 73.07 ($\pm$.45) & 68.69 ($\pm$.56) \\ 
RoBERTa-L \cite{roberta}(ours) &  72.17 ($\pm$.06) & 68.49 ($\pm$.07) \\
\midrule
% + RGCN\cite{rgcn}   & 72.69 & 68.41 \\
+ GconAttn \cite{DBLP:conf/aaai/WangKMYTACFMMW19} & 72.61 ($\pm$.39) & 68.59 ($\pm$.96) \\
+ KagNet \cite{DBLP:conf/emnlp/LinCCR19}   & 73.47 ($\pm$.22) & 69.01 ($\pm$.76) \\
% + RN\cite{DBLP:conf/nips/SantoroRBMPBL17}       & 74.57 & 69.08 \\
+ MHGRN \cite{DBLP:conf/emnlp/FengCLWYR20}   & 74.45 ($\pm$.10) & 71.11 ($\pm$.81)  \\
+ QA-GNN \cite{qagnn}   & 76.54 ($\pm$.21) & 73.41 ($\pm$.92) \\
\midrule
+ \textit{\textbf{\model}} & 73.76 ($\pm$.05) & 70.62 ($\pm$.07)\\ 
+ \textit{KGT-finetune} & 73.46 ($\pm$.07) & 70.04 ($\pm$.05)\\ 
+ \textit{KGT-scratch}  & 72.32 ($\pm$.05) & 69.18 ($\pm$.08)\\ 
\bottomrule
\end{tabular}
\label{tab:qa_eb}
% \vspace{-4mm}
% \end{wraptable}
\end{table}

==> tables/res-tc-error-ba.tex <==
\begin{table}[!hbpt]
% \begin{wraptable}{r}{0.6\textwidth}
    \centering
    % \vspace{-6mm}
     \caption{Results with error bar of triple classification on WN18RR\cite{rotate}.}
    \begin{tabular}{l|c c c c}
    \toprule
          & \textbf{Acc.} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}  \\
         \midrule
        TransE \cite{transe} &  88.35 & 93.45 & 82.48 & 87.62  \\ 
        RotatE \cite{rotate} & 88.26 & 93.03 & 82.71 & 87.57 \\
        ComplEx \cite{complex} & 85.07 & 96.73 & 72.59 & 82.94 \\
        \midrule
        \textit{\textbf{\model}}
        % \textbf{KGT}
        & 89.02$\pm$0.08 & 86.66$\pm$0.18 & 92.24$\pm$0.05 & 89.36$\pm$0.05 \\
        \textit{KGT-finetune} &  85.00$\pm$0.20 & 80.85$\pm$0.19 & 91.74$\pm$0.12 & 85.95$\pm$0.14 \\
        \textit{KGT-scratch} & 67.02$\pm$0.16 & 67.91$\pm$0.13 & 64.55$\pm$0.17 & 66.19$\pm$0.15 \\
        \bottomrule
    \end{tabular}
    \label{tab:tc_eb}
% \end{wraptable}
\end{table}

==> tables/res-zsl-error-bar.tex <==
\begin{table}[!hbpt]
% \begin{wraptable}{r}{0.55\textwidth}
    \centering
    \vspace{-3mm}
    \caption{Results with error bar of zero-shot image classification on AwA-KG\cite{k-zsl}}
    \begin{tabular}{l|c| c c c}
    \toprule
        %   \multirow{2}{*}{Method} & ZSL & \multicolumn{3}{c}{GZSL} \\
        % \cline{2-5}
          & \textbf{T1} & \textbf{S} & \textbf{U} & \textbf{H}    \\
         \midrule
        DeViSE\cite{devise} & 43.24 & 86.44 & 6.40 & 11.91  \\ 
        GCNZ\cite{gcnz}  & 62.98 & 75.59 & 20.28 & 31.98 \\
        OntoZSL\cite{ontozsl} & 62.65 & 59.59 & 50.58 & 54.71 \\
        \midrule
        \textit{\textbf{\model}} & 57.38$\pm$0.38 & 63.97$\pm$0.37 & 51.71$\pm$0.32 & 57.19$\pm$0.35 \\
        \textit{KGT-finetune} & 57.65$\pm$0.23 & 62.24$\pm$0.35 & 51.33$\pm$0.34 & 56.26$\pm$0.26 \\
        \textit{KGT-scratch} & 58.96$\pm$0.39 & 56.48$\pm$0.42 & 47.93$\pm$0.27 & 51.85$\pm$0.34 \\
        \bottomrule
    \end{tabular}
    \label{tab:zsl_eb}
    \vspace{-3mm}
% \end{wraptable}
\end{table}
